Transporting Causal Mechanisms for Unsupervised Domain Adaptation

Existing Unsupervised Domain Adaptation (UDA) literature adopts the covariate shift and conditional shift assumptions, which essentially encourage models to learn common features across domains. However, due to the lack of supervision in the target domain, they suffer from the semantic loss: the feature will inevitably lose non-discriminative semantics in source domain, which is however discriminative in target domain. We use a causal view -- transportability theory -- to identify that such loss is in fact a confounding effect, which can only be removed by causal intervention. However, the theoretical solution provided by transportability is far from practical for UDA, because it requires the stratification and representation of the unobserved confounder that is the cause of the domain gap. To this end, we propose a practical solution: Transporting Causal Mechanisms (TCM), to identify the confounder stratum and representations by using the domain-invariant disentangled causal mechanisms, which are discovered in an unsupervised fashion. Our TCM is both theoretically and empirically grounded. Extensive experiments show that TCM achieves state-of-the-art performance on three challenging UDA benchmarks: ImageCLEF-DA, Office-Home, and VisDA-2017. Codes are available in Appendix.

==> del_3_causal_view.tex <==
\section{Transportability View of DA}

Transportability theory~\cite{transportability} provides theoretical guidance to circumvent domain shift by transporting knowledge obtained in the source domain. To license such transport, one must establish assumptions on the ``mechanisms'' through which the domain differences arise.
We reformulate existing assumptions (\ie, covariate shift and conditional shift) into a more general one, and formally represent it as a Structural Causal Model (SCM)~\cite{xx}:
\begin{equation}
    \mathcal{M}:
    \begin{cases}
    X\leftarrow g(U, N_X),\\
    Y\leftarrow f(X, U, N_Y),\\
    U\leftarrow h^S(N_U^S),
    \end{cases}
\end{equation}
where $X$ denotes observation, $Y$ denotes the predicted label, $U$ denotes semantic attributes, $S\in\{0, 1\}$ is a selection variable to indicate domain ($S=0$ for source, $S=1$ for target), $f,g,h^0,h^1$ are functions and $N_X,N_Y,N_U^0,N_U^1$ are jointly independent exogenous noise variables. $\mathcal{M}$ is associated with a graphical model $\mathcal{G}$, called \emph{selection diagram}~\cite{xx}, as shown in Figure~\ref{fig:2}. The diagram is a directed acyclic graph, where nodes represent random variables, directed edges correspond to the functions in the SCM, and the selection variable $S$ specifies the ``mechanism'' that leads to domain shift. We will detail the edges in $\mathcal{G}$ (functions in $\mathcal{M}$) as follow:
% Selection diagram is a causal graph where nodes represent random variables and directed edges represent causal relations. It has a selection variable $S$ corresponding to the ``mechanism'' that leads to domain shift. Our selection diagram is shown in Figure~\ref{fig:2}, where $X$ denotes observation, $Y$ denotes the predicted label and $U$ denotes semantic attributes. The directed edges are as follows:

\noindent\textbf{$\mathbf{U}\to\mathbf{X}$}. The abstract, high-level semantic attribute $U$ generates the concrete, low-level observation $X$ (\eg, image). One can connect this with a conditional GAN~\cite{xx} taking attribute $U$ and noise variable $N_X$ as input to generate images. 
In fact, human commonly uses the reverse process $g^{-1}(X)$ to describe the observations (\eg, mattress image) with attributes (\eg patterned and rectangular).

\noindent\textbf{$\mathbf{U}\to\mathbf{Y},\mathbf{X}\to\mathbf{Y}$}. The first relation emulates how decomposed concepts define a class (\eg, rectangular shape$+$monochrome/patterned mattress$\to$``bed''). The second relation captures the effects towards prediction from discriminative details in observation $X$. The two links indeed coexist---such as human can predict the object label based solely on textual description of its attributes, or images showing its iconic features---hence the predictive function $f$ takes both $X,U$ as input.

\noindent\textbf{$\mathbf{S}\to\mathbf{U}$}. $S$ intervenes the structural assignment of the random variable $U$ such that $h^0 \neq h^1$ and/or $N_U^0 \neq N_U^1$, hence $P(U|S=0)\neq P(U|S=1)$, leading to domain differences. Note that while the distribution of $U$ differs across domains, the semantic attributes in $U$ are still meaningful in $S=0$ and $S=1$. This is because the source and target domain are deemed as related in real world DA tasks (otherwise nothing can be transported~\cite{xx}). 
% As shown later, this is an important basis to license transportability.
%This assumption is motivated by observing the properties of $g$ and $f$, which represents physical generative process of observation $X$ (from attribute $U$) and the defining characteristics of label $Y$ (\wrt $U$ and $X$). These are causal mechanisms that tend to stay invariant across domains~\cite{xxx}. Hence the domain shift can only originate from $U$, justifying $S\to U$. 

Our SCM $\mathcal{M}$ provides a general assumption on the domain shift in DA, and can cover the existing assumptions.

\noindent\textbf{$\mathcal{M}$ Covers Covariate and Conditional Shift}. First we will prove for conditional shift as covariate shift is a trivial case where $P(Y|X)$ is invariant across domains. The SCM $\mathcal{M}'$ for conditional shift is given below with its corresponding selection diagram $\mathcal{G}'$ shown in Figure 3.
\begin{equation}
    \mathcal{M'}:
    \begin{cases}
    X\leftarrow g_c(E_X),\\
    Y\leftarrow f_c^S(X, E_Y^{S}),
    \end{cases}
\end{equation}
where $g_c,f_c^0,f_c^1$ are functions and $E_X,E_Y^0,E_Y^1$ are noise variables (to differentiate from $\mathcal{M}$). Then $\mathcal{M}$ is a superset of $\mathcal{M}'$, \ie, for every SCM $M'\in\mathcal{M}'$, there exists a realization $M\in\mathcal{M}$ such that $M'=M$. Specifically, $M$ is given by: $N_X=E_X,N_Y=\varnothing,N_U^S=E_Y^S$ and $g(U,N_X)=g_c(N_X),f(X,U,N_Y)=f^{U_1}_c(X,U_2)),h^S(N_U^S):=(U_1,U_2)=(S,N_U^S)$. This can be understood intuitively from the graphical view in Figure 3, where $\mathcal{G}'$ corresponds to removing $U\to X$ and letting $U$ ``become'' $S$ in $\mathcal{G}$. In a similar fashion, covariate shift corresponds to removing $U\to Y$ and replacing $U$ with $S$. The detailed proof follows the analysis above and is included in the Appendix.

The goal of DA is to identify $P(Y|do(X),S)$, where $S=0$ in training and $S=1$ in testing. $do(X)$ represents causal intervention. In $\mathcal{M}$, $do(X=x)$ corresponds to replacing the structural assignment function of $X$ with $X\leftarrow x$. In $\mathcal{G}$, it corresponds to removing the link $U\to X$.
$P(Y|do(X),S)$ is equal to $P(Y|X)$ in the post-intervention population generated by the modified $\mathcal{M}$ and $\mathcal{G}$ in domain $S$, which removes the spurious confounding effect (\eg, predicting bed with background).
This is because in the post-intervention population, the generation of observation $X$ is no longer governed by $U$. Hence the data no longer contains spurious patterns caused by $U$ (\eg, all bed images have cluttered background).

However, in practice, we cannot directly evaluate $P(Y|do(X),S)$, as most datasets are generated from passive observation of the world, rather than actively intervening the physical generative process of observations. Fortunately, given a selection diagram, the transportability theory can reduce $P(Y|do(X),S)$ to a \emph{transport formula} containing measurable terms in $S=0$ and $S=1$. As formally proved in Appendix, the transport formula for $\mathcal{G}$ is given by Eq.~\eqref{eq:transportability}.

Based on this assumption, we have a solution to DA with theoretical guarantee. First mention the goal do(X), S. Why do(X)? What does S means? Introduce theorem 1: when is transport possible?

As formally shown in appendix, the transport formula is given by: ...
Training... Testing... 

This is a principled way to transport: it solve the semantic loss problem. Give example.

Mention the two problems.

==> tables/alpha_ablation.tex <==
\begin{table}[t!]
\centering
%\captionsetup{font=footnotesize,labelfont=footnotesize,skip=5pt}
\scalebox{0.9}{
\setlength\tabcolsep{1.5pt}
\begin{tabular}{p{1.0cm}<{\centering}p{1.1cm}<{\centering}p{1.1cm}<{\centering}p{1.1cm}<{\centering}p{1.1cm}<{\centering}p{1.1cm}<{\centering}p{1.1cm}<{\centering}p{0.6cm}}
%{cl|cccccc|cccccc}
\hline\hline
    $\alpha$ & I $\to$ P & P $\to$ I & I $\to$ C & C $\to$ I & C $\to$ P & P $\to$ C & Avg\\
\hline

    0.1 & 78.3 & 90.0 & 95.3 & 88.5 & 74.0 & 94.1 & 86.7\\
    
    0.5 & 79.2 & 92.0 & 96.7 & 91.5 & 78.0 & 95.5 & 88.8\\
    
    1.0 & 79.5 & 93.2 & 97.1 & 93.2 & 78.8 & 96.2 & 89.7\\
    
    4.0 & \textbf{79.9} & 94.1 & 97.6 & \textbf{93.8} & 79.6 & \textbf{96.9} & 90.3\\
    
    7.0 & 79.2 & \textbf{94.2} & \textbf{97.8} & \textbf{93.8} & \textbf{79.9} & 96.5 & 90.2\\
    
    10.0 & 78.8 & \textbf{94.2} & 97.3 & 93.3 & 79.3 & 96.5 & 90.0\\

\hline \hline
\end{tabular}}
\caption{Ablation on $\alpha$ in Eq. (8) with accuracy (\%) on the 6 UDA tasks from ImageCLEF-DA.}
\label{tab:alpha}
\vspace{-3mm}
\end{table}
